Calibrating Generative Flows through Regional Probability Matching

Generative models for scientific simulation must reproduce the frequencies of rare states as well as their structure. We developed generalized mass-preserving coupled flow matching (G-MPCF), which assigns regions of Gaussian noise the probability masses of corresponding regions in weighted observations. Conditional sampling within matched regions preserves the prescribed target distribution while changing the velocities used to train the flow, without modifying the underlying generative model architecture. On a rare-mode benchmark, an analytic coupling reduced relative score error by 95.0% and numerical integration error by 89.9% compared with independent pairing. On CIFAR-10 with a 100:1 class-probability ratio, G-MPCF reduced corrected class-mass error by 44.6% relative to minibatch optimal transport and improved mean image fidelity at matched computational budgets. These results show how the construction of training pairs can improve the reproduction of prescribed population frequencies by generative flows.

==> common/citation_numbers.tex <==
% Numbers in the single main reference list for the standalone supplement.
\makeatletter
\@namedef{b@sohl2015deep}{1}
\@namedef{b@ho2020denoising}{2}
\@namedef{b@song2019generative}{3}
\@namedef{b@song2021score}{4}
\@namedef{b@chen2018neural}{5}
\@namedef{b@grathwohl2019ffjord}{6}
\@namedef{b@papamakarios2021normalizing}{7}
\@namedef{b@duan2025reactot}{8}
\@namedef{b@li2024turbulence}{9}
\@namedef{b@hess2025downscaling}{10}
\@namedef{b@lipman2023flow}{11}
\@namedef{b@tong2024improving}{12}
\@namedef{b@albergo2023building}{13}
\@namedef{b@albergo2023stochastic}{14}
\@namedef{b@benamou2000computational}{15}
\@namedef{b@peyre2019computational}{16}
\@namedef{b@pooladian2023multisample}{17}
\@namedef{b@liu2023flow}{18}
\@namedef{b@kornilov2024optimal}{19}
\@namedef{b@chiang2026cotfm}{20}
\@namedef{b@chapel2025differentiable}{21}
\@namedef{b@lin2026modelaligned}{22}
\@namedef{b@grover2019bias}{23}
\@namedef{b@choi2020fair}{24}
\@namedef{b@sajjadi2018assessing}{25}
\@namedef{b@kynkaanniemi2019improved}{26}
\@namedef{b@naeem2020reliable}{27}
\@namedef{b@benton2024errorbounds}{28}
\@namedef{b@zhou2025erroranalysis}{29}
\@namedef{b@song2021ddim}{30}
\@namedef{b@lu2022dpmsolver}{31}
\@namedef{b@karras2022elucidating}{32}
\@namedef{b@song2023consistency}{33}
\@namedef{b@geng2025meanflow}{34}
\@namedef{b@bonneel2015sliced}{35}
\@namedef{b@heusel2017gans}{36}
\@namedef{b@he2016deep}{37}
\@namedef{b@deng2009imagenet}{38}
\@namedef{b@lloyd1982least}{39}
\@namedef{b@hairer1993solving}{40}
\@namedef{b@krizhevsky2009learning}{41}
\@namedef{b@ronneberger2015unet}{42}
\@namedef{b@wu2018group}{43}
\@namedef{b@loshchilov2019decoupled}{44}
\@namedef{b@gretton2012kernel}{45}
\@namedef{b@binkowski2018demystifying}{46}
\@namedef{b@parmar2022aliased}{47}
\@namedef{b@lipton2018detecting}{48}
\@namedef{b@vandermaaten2008visualizing}{49}
\@namedef{b@holm1979simple}{50}
\@namedef{b@efron1994introduction}{51}
\@namedef{b@tipping1999mixtures}{52}
\@namedef{b@clanuwat2018classical}{53}
\@namedef{b@reyes2013har}{54}
\@namedef{b@huang2026gmpcfdata}{55}
\makeatother

